Unsupervised Dense Information Retrieval with Contrastive Learning

Recently, information retrieval has seen the emergence of dense retrievers, using neural networks, as an alternative to classical sparse methods based on term-frequency. These models have obtained state-of-the-art results on datasets and tasks where large training sets are available. However, they do not transfer well to new applications with no training data, and are outperformed by unsupervised term-frequency methods such as BM25. In this work, we explore the limits of contrastive learning as a way to train unsupervised dense retrievers and show that it leads to strong performance in various retrieval settings. On the BEIR benchmark our unsupervised model outperforms BM25 on 11 out of 15 datasets for the Recall@100. When used as pre-training before fine-tuning, either on a few thousands in-domain examples or on the large MS~MARCO dataset, our contrastive model leads to improvements on the BEIR benchmark. Finally, we evaluate our approach for multi-lingual retrieval, where training data is even scarcer than for English, and show that our approach leads to strong unsupervised performance. Our model also exhibits strong cross-lingual transfer when fine-tuned on supervised English data only and evaluated on low resources language such as Swahili. We show that our unsupervised models can perform cross-lingual retrieval between different scripts, such as retrieving English documents from Arabic queries, which would not be possible with term matching methods.

==> ablations.tex <==
\section{Ablation studies}

% Pre-training setup:
% \begin{itemize}
% \item MoCo vs SimCLR (questions: is momentum useful? performance wrt queue size?)
% \item BERT vs no BERT
% \item Data augmentations (cropping, ICT, word masking/deleting, shuffling)
% \item CLS token vs averaging, training data (ccnet, trec-covid, etc), size of vocab
% \end{itemize}

In this section, we investigate the influence of different design choices of the method used in the previous section.
For these experiments, we use a reduced setting, where the model is pre-trained for 200,000 gradient steps, with a batch size of 2,048 (over 32 GPUs) on Wikipedia.
For the fine-tuning on MS MARCO, the model is trained on 8 GPUs with a batch size of $512$ for 20,000 gradient steps with the AdamW optimizer, without hard negatives.
%\eg{should we only report results after fine-tuning on MS MARCO? It will make the discussion simpler, and this is probably still the main use case of the paper}

%In this subsection we investigation the influence of different components of the method used in the previous sections. For this we use a minimal setting, where the model is pretrained for 200k gradient steps on 32 gpus, for the finetuning phase on MSMarco the model is trained using 8 gpus during 20k gradients steps without hard negatives. The hyperparameters used here can be found in Table~\ref{tab:hyperparameters}.

\begin{figure}[t]
    \centering
    \includegraphics{queue_size.pdf}
    \caption{\textbf{Queue size.} We report nDCG@10 before and after fine-tuning on MS MARCO.
    \aj{same for simclr?}}
    \label{fig:queue_size}
\end{figure}

\subsection{MoCo vs. SimCLR}
First, we compare the two contrastive pre-training methods: MoCo and SimCLR.
As in SimCLR, the number of negative examples is equal to the batch size, we train models with a batch size of \textcolor{red}{4,096} and restrict the queue in MoCo to the same number of elements.
Thus, in this experiments, we investigate the effect of using of momentum encoder for the keys, instead of backpropagating the gradient and using stochastic gradient descent.
We report results, with and without fine-tuning on MS MARCO in Table~\ref{tab:simclr_vs_moco}.
We observe that the difference between the two methods is not important, especially after training on MS MARCO.
Thus, we propose to use MoCo as it will allow to easily scale the number of negative examples used to train the model, an important ingredient for contrastive learning.
\eg{We need to re-run either SimCLR w/ batch size 2,048 or MoCo w/ batch size 4,096.}

\begin{table*}[h]
  \center
  \small
  \begin{tabular}{l ccccccccc}
    \toprule
           & NFCorpus  & NQ   & FiQA & ArguAna & Quora & DBPedia & SciDocs & FEVER & AVG \\
    \midrule
    %MoCo   & 25.9 & 13.1 & 12.9 & 32.8 & 69.0 & 18.9 & 12.2 & 56.8 & 29.9 \\
    %SimCLR & 24.2 & 21.6 & 13.0 & 33.7 & 74.9 & 17.9 & 13.6 & 56.1 & 31.9 \\
    %\midrule
    MoCo   & 31.1 & 37.2 & 23.4 & 41.6 & 82.7 & 36.9 & 15.7 & 71.5 & 41.5 \\
    SimCLR & 29.6 & 36.5 & 23.3 & 38.6 & 83.6 & 34.4 & 16.2 & 72.3 & 41.8 \\
    \bottomrule
  \end{tabular}
  \label{tab:simclr_vs_moco}
  \caption{\textbf{MoCo vs. SimCLR.} In this table, we report nDCG@10 on the BEIR benchmark for SimCLR and MoCo, after fine-tuning on the MS MARCO dataset.}
\end{table*}

\subsection{Queue size}
Next, we study the influence of the number of negatives used in the contrastive loss, by varying the queue size of the MoCo algorithm.
We consider values ranging from 2,048 to 131,072, and report results in Figure~\ref{fig:queue_size}.
We see that on average over the BEIR benchmark, increasing the number of negatives leads to better retrieval performance, especially in the unsupervised setting.
However, it is interesting to note that this effect is not equally strong for all datasets.

%\gi{Would be better with something similar with simclr?}

%The use of a queue without backpropagation allows us to easily scale the size of the pool of negatives. As shown in Table~\ref{tab:queue_size}, scaling the queue size improves both the zero-shot performance and the performance after finetuning on MSMarco.

\subsection{Data augmentations}
Third, we compare different ways to generate pairs of positive examples from a single document or chunk of text.
In particular, we compare random cropping, which leads to pairs with overlap, and the inverse cloze task, which was previously considered to pre-train retrievers.
Interestingly, as shown in Table~\ref{tab:data_augmentation}, the random cropping strategy strongly outperforms the inverse cloze task.
We argue that overlap between the two views of the data is beneficial, as it allows the network to learn lexical matching, similarly to BM25.
We also investigate whether additional data perturbations, such as random word deletion or replacement, are beneficial for retrieval.
After fine-tuning on MS MARCO, it seems that such data perturbations slightly degrade the performance of dense retrievers.

\begin{table*}[h]
  \center
  \small
  \begin{tabular}{l ccccccccc}
    \toprule
    & NFCorpus & NQ & ArguAna & Quora & DBPedia & SciDocs & FEVER & Overall \\
    \midrule
    ICT             & 30.5 & 37.5 & 32.6 & 82.3 & 33.1 & 14.6 & 67.9 & 39.5 \\
    Crop            & 31.5 & 44.1 & 39.5 & 84.2 & 39.6 & 16.3 & 74.8 & 44.3 \\ % 46005732 - moco - qsize 65536 - ratio 10-50% 256 tokens
    Crop + delete   & 31.6 & 42.3 & 39.2 & 84.6 & 39.7 & 16.2 & 71.8 & 43.4 \\ % 46211625 - moco - delete 10% - qsize 65536 - ratio 10-50% 256 tokens
    Crop + replace  & 30.5 & 43.2 & 42.6 & 84.6 & 39.2 & 16.0 & 73.8 & 43.6 \\ % 46211626 - moco - replace 10% - qsize 65536 - ratio 10-50% 256 tokens
    \bottomrule
  \end{tabular}
  \caption{\textbf{Data augmentions.} We report nDCG@10 after fine-tuning on MS MARCO.}
  \label{tab:data_augmentation}
\end{table*}


%Data augmentations are key component of contrastive learning methods used in computer vision, in the main results presented in this paper we do a very minimal use of them. In Table~\ref{tab:augmentations} we consider different data augmentation strategies. Namely we present results with random deletion, random token replacement and random masking of p\% of the tokens. Additionally we consider cropping with and without overlap. 

\subsection{Training data}
Finally, we study the impact of the pre-training data on the performance of our retriever, by training on Wikipedia, CCNet or a mix of both sources of data.
We report results in Table~\ref{tab:training_data}, and observe that there is no clear winner between the two data sources.
Unsurprisingly, pre-training on Wikipedia leads to better performance on datasets for which documents also come from Wikipedia, such as NaturalQuestions or FEVER.
On the other hand, on datasets from different domains than Wikipedia such as FiQA or ArguAna, training on the more diverse CCNet data leads to better results.
To get the best of both worlds, we consider to strategies to mix the two data sources.
In the 50/50\% strategy, examples are sampled uniformly across domain, meaning that half the batches are from Wikipedia and the other half from CCNet.
In the uniform strategy, examples are sampled uniformly over the union of the dataset.
Since CCNet is significantly larger than Wikipedia, this means that most of the batches are from CCNet.

\begin{table*}[h]
  \center
  \small
  \begin{tabular}{l cccccccccccccc}
    \toprule
           & NFCorpus & NQ & FiQA & ArguAna & Quora & DBPedia & SciDocs & FEVER & Overall \\
    \midrule
    %Wiki          & 27.6 & 17.7 & 35.6 & 75.4 & 21.0 & 13.3 & 64.5 & 63.0 & 33.0 \\ % 46005732 - moco - qsize 65536 - ratio 10-50% 256 tokens
    %CCNet         & 29.5 & 25.8 & 35.2 & 80.6 & 20.5 & 14.9 & 60.9 & 59.4 & 34.9 \\ % 46307600 - moco - cc-net - qsize 65536 - m=0.999
    %50/50\%       & 27.1 & 17.8 & 39.1 & 76.5 & 19.9 & 13.9 & 66.3 & 66.0 & 34.7 \\ % 46403749 - moco - 50-50 cc-net/wiki - lr 7e-5 - qsize 65536 - m=0.999
    %Uniform       & 29.1 & 19.2 & 36.2 & 79.0 & 22.6 & 13.6 & 64.0 & 62.7 & 35.6 \\ % 46435971 - moco - uniform cc-net/wiki - lr 7e-5 - qsize 65536 - m=0.999
    %\midrule
    Wiki          & 31.5 & 44.1 & 26.8 & 39.5 & 84.2 & 39.6 & 16.3 & 74.8 & 44.3 \\
    CCNet         & 31.8 & 39.9 & 31.6 & 43.3 & 84.5 & 36.1 & 16.0 & 66.4 & 42.4 \\
    50/50\%       & 31.7 & 43.2 & 27.1 & 35.9 & 84.7 & 39.5 & 15.8 & 77.4 & 44.0 \\
    Uniform       & 32.0 & 41.5 & 30.5 & 39.9 & 84.9 & 39.6 & 16.2 & 72.0 & 44.1 \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Training data.} We report nDCG@10 after fine-tuning on MS MARCO.}
  \label{tab:training_data}
\end{table*}



==> tables/queue_size.tex <==
\begin{table*}[t!]
  \small
  \center
  \begin{tabular}{@{}l  c c c c c c c @{}}
    \toprule
    \textbf{Queue size} & 2k & 4k & 8k & 16k & 32k & 64k & 128k \\
    \midrule
    MSMARCO       & 12.6 & 12.7 & 14.1 & 14.9 & & 15.6 \\
    TREC-COVID    & 21.8 & 24.8 & 22.8 & 23.9 & & 21.7 \\
    NFCorpus      & 23.4 & 25.9 & 27.6 & 26.6 & & 27.6 \\
    NQ            & 11.6 & 13.1 & 13.5 & 15.4 & & 17.7 \\
    HotpotQA      & 31.2 & 35.5 & 38.5 & 39.7 & & 44.9 \\
    FiQA-2018     & 12.8 & 12.9 & 13.6 & 16.8 & & 16.3 \\
    ArguAna       & 32.6 & 32.8 & 30.1 & 33.2 & & 35.6 \\
    T\'ouche-2020 & 11.8 & 12.8 & 11.2 & 14.0 & & 13.5 \\
    Quora         & 67.8 & 69.0 & 72.1 & 72.9 & & 75.4 \\
    DBPedia       & 15.3 & 18.9 & 18.6 & 19.4 & & 21.0 \\
    SCIDOCS       & 11.3 & 12.2 & 12.7 & 12.8 & & 13.3 \\
    FEVER         & 54.9 & 56.8 & 58.9 & 63.0 & & 64.5 \\
    Climate-FEVER & 11.6 & 14.3 & 12.4 & 16.1 & & 14.4 \\
    SciFact       & 58.8 & 60.3 & 59.6 & 63.0 & & 63.0 \\
    \midrule
    AVERAGE       & 28.1 & 29.9 & 30.1 & 32.0 & & 33.0 \\
    \bottomrule
  \end{tabular}
  \caption{Zero-shot NDCG@10 depending on the queue size.}
  \label{tab:ndcg_zs_queue_size}
\end{table*}

\begin{table*}[t!]
  \small
  \center
  \begin{tabular}{@{}l  c c c c c c c @{}}
    \toprule
    \textbf{Queue size} & 2k & 4k & 8k & 16k & 32k & 64k & 128k \\
    \midrule
    MSMARCO       & 29.5 & 30.0 & 30.1 & 30.1 & & 30.7 \\
    TREC-COVID    & 40.1 & 38.4 & 37.9 & 40.9 & & 41.7 \\
    NFCorpus      & 30.9 & 31.1 & 31.6 & 31.1 & & 31.0 \\
    NQ            & 37.6 & 37.2 & 37.5 & 37.0 & & 39.7 \\
    HotpotQA      & 60.8 & 61.7 & 62.5 & 62.7 & & 64.4 \\
    FiQA-2018     & 23.4 & 23.4 & 23.1 & 24.6 & & 25.0 \\
    ArguAna       & 42.1 & 41.6 & 41.6 & 40.3 & & 41.3 \\
    T\'ouche-2020 & 14.1 & 13.3 & 13.1 & 15.3 & & 13.7 \\
    Quora         & 83.0 & 82.7 & 83.2 & 83.5 & & 83.9 \\
    DBPedia       & 34.0 & 36.9 & 36.8 & 37.9 & & 38.5 \\
    SCIDOCS       & 15.1 & 15.7 & 16.2 & 16.0 & & 15.9 \\
    FEVER         & 71.5 & 71.5 & 72.2 & 73.8 & & 74.7 \\
    Climate-FEVER & 18.1 & 19.3 & 18.8 & 19.2 & & 18.0 \\
    SciFact       & 64.1 & 66.3 & 67.3 & 67.2 & & 66.4 \\
    \midrule
    AVERAGE       & 41.1 & 41.5 & 41.7 & 42.3 & & 42.6 \\
    \bottomrule
  \end{tabular}
  \caption{Zero-shot NDCG@10 depending on the queue size, after training on MS MARCO.}
  \label{tab:ndcg_msmarco_queue_size}
\end{table*}











\begin{table*}[t!]
    \small
    \center
    \begin{tabular}{@{}l  c c c c c c c @{}}
        \toprule
        \textbf{Queue size} & $2^{11}$ & $2^{12}$ & $2^{13}$ & $2^{14}$ & $2^{15}$ & $2^{16}$ & $2^{17}$ \\
        \midrule
   MSMARCO       & 12.6	& 12.7 & \\
   TREC-COVID    & 21.8 & \\
   NFCorpus      & 23.4 & \\
   NQ            & 11.6 & \\
   HotpotQA      & 31.2 & \\
   FiQA-2018     & 12.8 & \\
   ArguAna       & 32.6 & \\
   T\'ouche-2020 & 11.8 & \\
   Quora         & 67.8 & \\
   DBPedia       & 15.3 & \\
   SCIDOCS       & 11.3 & \\
   FEVER         & 54.9 & \\
   Climate-FEVER & 11.6 & \\
   SciFact       & 58.8 & \\
   \midrule
   AVERAGE       &  \\
   \bottomrule
    \end{tabular}
    \caption{Zero-shot NDCG@10 depending on the queue size.}
    \label{tab:ndcg_zs_queue_size}
\end{table*}

\begin{table*}[t!]
    \small
    \center
    \begin{tabular}{@{}l  c c c c c c c @{}}
        \toprule
        \textbf{Queue size} & $2^{11}$ & $2^{12}$ & $2^{13}$ & $2^{14}$ & $2^{15}$ & $2^{16}$ & $2^{17}$ \\
        \midrule
   MSMARCO       & \\
   TREC-COVID    & \\
   NFCorpus      & \\
   NQ            & \\
   HotpotQA      & \\
   FiQA-2018     & \\
   ArguAna       & \\
   T\'ouche-2020 & \\
   Quora         & \\
   DBPedia       & \\
   SCIDOCS       & \\
   FEVER         & \\
   Climate-FEVER & \\
   SciFact       & \\
   \midrule
   AVERAGE       &  \\
   \bottomrule
    \end{tabular}
    \caption{Zero-shot NDCG@10 depending on the queue size.}
    \label{tab:recall_zs_queue_size}
\end{table*}


==> tables/recall_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t!]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{@{}l  cc cc cc cc >{\columncolor{bluegrey}}c} 
 \toprule
 %\multicolumn{10}{@{}c@{}}{\bf nDCG@10}\\
 %\midrule
 & BM25 & ColBERT &  SPARTA & docT5Query & DPR & ANCE & GenQ & TAS-B & Ours \\
 \midrule
    %MS MARCO & 65.8 & 86.5 & 79.3 & 81.9 & 55.2 & 85.2 & 88.4 & 88.4 & 89.1 \\
    TREC-COVID & 49.8 & 46.4 & 40.9 & \bf 54.1 & 21.2 & 45.7 & 45.6 & 38.7 & 40.7 \\
    NFCorpus & 25.0 & 25.4 & 24.3 & 25.3 & 20.8 & 23.2 & 28.0 & 28.0 & \bf 30.0 \\
    NQ & 76.0 & 91.2 & 78.7 & 83.2 & 88.0 & 83.6 & 86.2 & 90.3 & \bf 92.5 \\
    HotpotQA & 74.0 & 74.8 & 65.1 & 70.9 & 59.1 & 57.8 & 67.3 & 72.8 & \bf 77.7 \\
    FiQA & 53.9 & 60.3 & 44.6 & 59.8 & 34.2 & 58.1 & 61.8 & 59.3 & \bf 65.6 \\
    ArguAna & 94.2 & 91.4 & 89.3 & 97.2 & 75.1 & 93.7 & \bf 97.8 & 94.2 & 97.7 \\
    Touch\'e-2020 & 53.8 & 43.9 & 38.1 & \bf 55.7 & 30.1 & 45.8 & 45.1 & 43.1 & 29.4 \\
    CQADupStack & 60.6 & 62.4 & 52.1 & 63.8 & 40.3 & 57.9 & 65.4 & 62.2 & \bf 66.3 \\
    Quora & 97.3 & 98.9 & 89.6 & 98.2 & 47.0 & 98.7 & 98.8 & 98.6 & \bf 99.3 \\
    DBPedia & 39.8 & 46.1 & 41.1 & 36.5 & 34.9 & 31.9 & 43.1 & 49.9 & \bf 54.1 \\
    SCIDOCS & 35.6 & 34.4 & 29.7 & 36.0 & 21.9 & 26.9 & 33.2 & 33.5 & \bf 37.8 \\
    FEVER & 93.1 & 93.4 & 84.3 & 91.6 & 84.0 & 90.0 & 92.8 & 93.7 & \bf 94.9 \\
    Climate-FEVER & 43.6 & 44.4 & 22.7 & 42.7 & 39.0 & 44.5 & 45.0 & 53.4 & \bf 57.4 \\
    SciFact & 90.8 & 87.8 & 86.3 & 91.4 & 72.7 & 81.6 & 89.3 & 89.1 & \bf 94.7 \\
 \midrule
 Avg. & 63.4 & 64.3 & 56.2 & 64.7 & 47.7 & 60.0 & 64.2 & 64.8 & \bf 67.0\\
 Best on  & 0 & 0 & 0 & 2 & 0 & 0 & 1 & 0 & \bf 11 \\
\bottomrule
\end{tabular}
\caption{\textbf{BEIR Benchmark.} 
  We report Recall@100 on the test sets of the datasets from the BEIR benchmark for bi-encoder methods without re-ranker.
  We also report the average (``Avg.'') and number of datasets where a method is the best (``Best on'') over the entire BEIR benchmark (excluding three datasets because of their licence).
  We evaluate retrievers after pre-training on unsupervised data with our contrastive learning and finetuning on MS-MARCO (``Ours'').
  Bold is the best overall.
  %
}
\label{tab:beir_recall}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tables/zeroshot.tex <==
\begin{table*}[t!]
    \centering
    \begin{tabular}{l | c c c c c}
        \toprule
        %Datasets & BM25 & Bert (Avg. repr. - cos. sim.) & SBert (cos. sim.) & MoCo \\
        Datasets & BM25 & Bert & SBert & MoCo (500k) & MoCo w/oBERT (200k) \\
        \midrule
   MSMARCO       & 0.218 & & & 0.168 & 0.170 \\ \midrule
   TREC-COVID    & 0.616 & 0.095 & 0.429 & 0.175 & 0.372 \\
   NFCorpus      & 0.297 & 0.027 & 0.213 & 0.293 & 0.270 \\ \midrule
   NQ            & 0.753 & 0.027 & 0.244 & 0.188 & 0.204 \\ 
   HotpotQA      & 0.601 & 0.052 & 0.286 & 0.406 & 0.483 \\ 
   FiQA-2018     & 0.239 & 0.012 & 0.147 & 0.181 & 0.149 \\ \midrule
   ArguAna       & 0.441 & 0.237 & 0.345 & 0.400 & 0.389 \\
   T\'ouche-2020 & 0.605 & 0.025 & 0.174 & 0.120 & 0.218 \\ \midrule 
   Quora         & 0.742 & 0.478 & 0.831 & 0.737 & 0.678 \\ \midrule
   DBPedia       & 0.288 & 0.036 & 0.249 & 0.220 & 0.320 \\ \midrule
   SCIDOCS       & 0.156 & 0.023 & 0.096 & 0.145 & 0.134 \\ \midrule
   FEVER         & 0.648 & 0.045 & 0.258 & 0.595 & 0.606 \\ 
   Climate-FEVER & 0.179 & 0.027 & 0.137 & 0.144 & 0.144 \\ 
   SciFact       & 0.620 & 0.067 & 0.323 & 0.669 & 0.630 \\ \midrule
   AVERAGE       &  \\ 
        \bottomrule
    \end{tabular}
    \caption{Zero-shot retrieval performance on \beir datasets. Scores denote \textbf{NDCG@10}.}
    \label{tab:results-recall}
\end{table*}


\begin{table*}[t!]
    \centering
    \begin{tabular}{l | c c c c c }
        \toprule
        Datasets & BM25 & Bert & SBert & MoCo & MoCo w/o Bert \\
        \midrule
   MSMARCO       & 0.621 & & 0.546 & 0.609 & 0.581 \\ \midrule
   TREC-COVID    & 0.447 & & & \\
   NFCorpus      & 0.196 & 0.058 & 0.213 & 0.271 & 0.246 \\ \midrule
   NQ            & 0.753 & 0.130 & 0.669 & 0.693 & 0.707 \\ 
   HotpotQA      & 0.757 & 0.161 & 0.488 & 0.622 & 0.684 \\ 
   FiQA-2018     & 0.505 & 0.065 & 0.414 & 0.457 & 0.406 \\ \midrule
   ArguAna       & 0.931 & 0.591 & 0.919 & 0.934 & 0.897 \\  
   T\'ouche-2020 & 0.463 & 0.028 & 0.216 & 0.207 & 0.247 \\ \midrule 
   Quora         & 0.948 & 0.746 & 0.982 & 0.962 & 0.946 \\ \midrule
   DBPedia       & 0.384 & 0.080 & 0.340 & 0.382 & 0.404 \\ \midrule
   SCIDOCS       & 0.346 & 0.101 & 0.269 & 0.373 & 0.322 \\ \midrule
   FEVER         & 0.908 & 0.108 & 0.550 & 0.919 & 0.918 \\ 
   Climate-FEVER & 0.383 & 0.086 & 0.405 & 0.450 & 0.467 \\ 
   SciFact       & 0.838 & 0.354 & 0.659 & 0.945 & 0.915 \\ \midrule
   AVERAGE       \\ 
        \bottomrule
    \end{tabular}
    \caption{Zero-shot retrieval performance on \beir datasets. Scores denote \textbf{Recall@100}.}
    \label{tab:results-recall}
\end{table*}
